Shifting to Machine Supervision: Annotation-Efficient Semi and Self-Supervised Learning for Automatic Medical Image Segmentation and Classification

Advancements in clinical treatment are increasingly constrained by the limitations of supervised learning techniques, which depend heavily on large volumes of annotated data. The annotation process is not only costly but also demands substantial time from clinical specialists. Addressing this issue, we introduce the S4MI (Self-Supervision and Semi-Supervision for Medical Imaging) pipeline, a novel approach that leverages advancements in self-supervised and semi-supervised learning. These techniques engage in auxiliary tasks that do not require labeling, thus simplifying the scaling of machine supervision compared to fully-supervised methods. Our study benchmarks these techniques on three distinct medical imaging datasets to evaluate their effectiveness in classification and segmentation tasks. Notably, we observed that self supervised learning significantly surpassed the performance of supervised methods in the classification of all evaluated datasets. Remarkably, the semi-supervised approach demonstrated superior outcomes in segmentation, outperforming fully-supervised methods while using 50% fewer labels across all datasets. In line with our commitment to contributing to the scientific community, we have made the S4MI code openly accessible, allowing for broader application and further development of these methods.

==> extra.tex <==
\begin{figure}[!h]
\begin{minipage}[t]{0.5\linewidth}
    \centering
    \includegraphics[width=1\textwidth]{image/dermofit_data.png}
\end{minipage}
\hspace{0.55cm}
\begin{minipage}[t]{0.5\linewidth} 
    \centering
    \includegraphics[width=1\textwidth]{image/dermofit_gt.png}
\end{minipage}       
\hspace{0.55cm}
\begin{minipage}[t]{0.5\linewidth} 
    \centering
    \includegraphics[width=1\textwidth]{image/dermofit_pred.png}
\end{minipage}  
\caption{Dermofit dataset visualization, top left: data (input image), top right: mask (label image), bottom left: prediction image}
\label{fig:dermofit_data}
\end{figure} 

\begin{figure}[!h]
\begin{minipage}[t]{0.5\linewidth}
    \centering
    \includegraphics[width=1\textwidth]{image/isic_data.png}
\end{minipage}
\hspace{0.55cm}
\begin{minipage}[t]{0.5\linewidth} 
    \centering
    \includegraphics[width=1\textwidth]{image/isic_label.png}
\end{minipage}       
\hspace{0.55cm}
\begin{minipage}[t]{0.5\linewidth} 
    \centering
    \includegraphics[width=1\textwidth]{image/isic_pred.png}
\end{minipage} 
\caption{ISIC2017 dataset visualization, top left: data (input image), top right: mask (label image), bottom left: prediction image}
\label{fig:isic_data}
\end{figure} 
\begin{figure}[!h]
\begin{minipage}[t]{0.5\linewidth}
    \centering
    \includegraphics[width=1\textwidth]{image/Dermatomyositis_data.png}
\end{minipage}
\hspace{0.55cm}
\begin{minipage}[t]{0.5\linewidth} 
    \centering
    \includegraphics[width=1\textwidth]{image/Dermatomyositis_label.png}
\end{minipage}       
\hspace{0.55cm}
\begin{minipage}[t]{0.5\linewidth} 
    \centering
    \includegraphics[width=1\textwidth]{image/Dermatomyositis_pred.png}
\end{minipage} 
\caption{Dermatomyositis dataset visualization, top left: data (input image), top right: mask (label image), bottom left: prediction image}
\label{fig:Dermatomyositis_data}
\end{figure} 

\paragraph{Data Imbalances and Weight Initializations:} For each of our datasets, there are a lot more background pixels (area out of interest) as opposed to the foreground pixels (area of interest). %Due to the fact that the dataset only partially contains cells (Dermatomyositis) or skin lesion (Dermofit, ISIC2017), and a larger portion of each image consist of a blank area that is out of interest, we consider the three datasets to be unbalanced in pixel level. 
The Dermatomyositis dataset has a background-to-target ratio is 0.8521 to 0.1479; the Dermofit Background to target ratio is 0.6963 to 0.3037; and ISIC2017 has a background-to-target ratio is 0.7980 to 0.2020. 
To counter the impact that the background might have on the loss function (hence model preference in optimization and prediction), we initialize the cross-entropy loss by these values in each case.  

Besides using the pixel weight, we also test another weight initialization (median frequency weight\cite{DBLP:journals/corr/EigenF14}). 
Namely, the median frequency weight received by each class is derived from the reciprocal of the pixel ratio of a particular class, normalized by the median frequency of the class\cite{liu2019deepcrack, liu2019roadnet} as mentioned in Table \ref{table:weight_table}.

%%%%%%%%%%% PicIE table
\begin{table}[!h]
    \centering
    \caption{Performance Analysis for the Unsupervised PiCIE approach. mIOU stands for mean intersection over union.}
    \begin{tabular}{cccccccc}
        \toprule
         {\textbf{Dataset}} & {\textbf{ResNet}} & { \textbf{mIOU} } \\
        \midrule
        {\textbf{Dermofit}} & ResNet34  & 0.5698 $\pm$ 0.028 \\
        \midrule
        {\textbf{Dermatomyositis}} & ResNet34  & 0.4151 $\pm$ 0.038 \\
        \midrule
        {\textbf{ISIC2017}} & ResNet34 &  0.4514 $\pm$ 0.045 \\
        \bottomrule
    \end{tabular} 
    \label{table:PiCIE_performance}
\end{table}


\subsection{Comparing DEDL\cite{singh2022dataefficient} and the Semi-supervised cross teaching approach \cite{luo2021ctbct} for Segmentation}\label{subsec1}

In Table \ref{table: fullyvsSemi}, we compare the auto-encoder post-processing based DEDL \cite{singh2022dataefficient} with the semi-supervised cross-teaching based approach by \citet*{luo2021ctbct} over four different label fractions - 10\%, 50\%, 70\%, and 100\%. When we say the architecture is trained with x\% label fraction, the architecture had access to only x\% of the total labeled image dataset and not per image. For a fair comparison, we compare the Swin-Transformer trained by the Semi-supervised cross-teaching approach \cite{luo2021ctbct} and the ResNet-34 trained U-Net by DEDL \cite{singh2022dataefficient}. In almost all scenarios, the cross-teaching semi-supervised approach performs better than DEDL. This also aligns without intuition, as during training for each epoch and each batch, the semi-supervised approach also learned from the unlabeled data.

\begin{figure}[ht]
    \centering
    \includegraphics[width=1\textwidth]{image/unsupervised.png}
    \caption{Unsupervised Segmentation Approach: PiCIE pipeline image from \cite{picie2021}. $View_1$ and $View_2$ (at the bottom) represent two photometrically transformed views of the input image, whereas $View_1$ and $View_2$ (at the top) represent the geometric transformation of one of the views.} % Should add more detail in caption
    \label{fig:picie_fig}
\end{figure}



\begin{table}[!htbp] 
    \caption{Comparison Between Fully- VS Semi-Supervised Models} 
        \begin{tabular}{c|cccccc}
            \toprule
             & \multicolumn{5}{c}{ \textbf{Percentage of Training data ($x \%$ labeled data)} } \\
             &$0 \%$  & $10 \%$  & $50 \%$  & $70 \%$ & $100 \%$  \\
            
            \midrule
             & \multicolumn{4}{c}{ \textbf{Dermofit Dataset (Interpolate to 480x480 then resize to 224x224)}} \\
            \midrule
            \textbf{PiCIE(Rn34)} &0.5698 $\pm$ 0.028 &&&& \\
            \textbf{DEDL(Rn34)} & &0.6599 $\pm$ 0.015 & 0.7198 $\pm$ 0.02 & 0.7229 $\pm$ 0.013 & 0.7576 $\pm$ 0.01 \\
            \textbf{Semi-SL(ST)} & &\textbf{0.7244 $\pm$ 0.0096} & \textbf{0.7954 $\pm$ 0.0027} & \textbf{0.8033 $\pm$ 0.0044} & \textbf{0.8182 $\pm$ 0.0002} \\
            % \textbf{SSL(Unet)} & 1 & 1 & 1 & 1\\
            
            \midrule  
             & \multicolumn{4}{c}{ \textbf{Dermatomyositis (Tilling to 480x480 then resize to 224x224) }} \\
            \midrule
            \textbf{PiCIE(Rn34)} &0.4151 $\pm$ 0.038 &&&& \\
            \textbf{DEDL(Rn34)} & &0.4237 $\pm$ 0.013 & 0.5261 $\pm$ 0.0150 & 0.5407 $\pm$ 0.0180 & 0.5306 $\pm$ 0.0230 \\
            \textbf{Semi-SL(ST)} & &\textbf{0.5106 $\pm$ 0.0067} & \textbf{0.5338 $\pm$ 0.00171} & \textbf{0.555 $\pm$ 0.0009} & \textbf{0.5751 $\pm$ 0.0025} \\
             
             \midrule
             & \multicolumn{4}{c}{ \textbf{ISIC-2017 (Interpolate to 480x480 then resize to 224x224) }} \\
            \midrule
            \textbf{PiCIE(Rn34)} &0.4514 $\pm$ 0.045 &&&& \\
            \textbf{DEDL(Rn34)} & &\textbf{0.5857 $\pm$ 0.014} & 0.6171 $\pm$ 0.01 & 0.5951 $\pm$ 0.053 & 0.6518 $\pm$ 0.013 \\
            \textbf{Semi-SL(ST)} & &0.5712 $\pm$ 0.014 & \textbf{0.6637 $\pm$ 0.017} & \textbf{0.6763 $\pm$ 0.027} & \textbf{0.7062 $\pm$ 0.02} \\
            % \textbf{SSL(Unet)}      & 0.5174 $\pm$ 0.019 & 0.5543 $\pm$ 0.0284 & 0.5521 $\pm$ 0.0167 & 0.5456 $\pm$ 0.0134 \\
            \bottomrule
        \end{tabular}
        \caption{Comparison Between Fully, Semi and UnSupervised architectures. Here Rn34 represents ResNet-34 while ST represents Swin-U-Net. Since \cite{picie2021} is an unsupervised approach, it does not require any labels for fine-tuning. Hence we present results for PiCIE using ResNet-34 backbone under 0\% label fractions. } 
    \label{table: fullyvsSemi}
\end{table}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{lllll}
\midrule
\textbf{Backbone}          & \textbf{Technique}                                           & \textbf{\begin{tabular}[c]{@{}l@{}}Autoimmune Dataset\\ F1 Score\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Dermofit Dataset\\ F1 Score\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}ISIC 2017 Dataset\\ Recall Score\end{tabular}} \\
\midrule
\multirow{3}{*}{ResNet-50} & DINO                                                         & 0.84252±0.008                                                                  & 0.6775±0.0005                                                                & \textbf{0.7407±0.0363}                                                                 \\
                           & CASS                                                         & \textbf{0.8650±0.0001}                                                                 & \textbf{0.7132±0.0003}                                                              & 0.699±0.0304                                                                  \\
                           & \begin{tabular}[c]{@{}l@{}}ImageNet \\ Transfer\end{tabular} & 0.83895±0.007                                                                  & 0.6341±0.0077                                                                & 0.6774±0.0004                                                                 \\
\midrule
\multirow{3}{*}{ViT B16}   & DINO                                                         & 0.8639± 0.002                                                                  & 0.4810±0.0012                                                                & 0.6571± 0.076                                                                 \\
                           & CASS                                                         & \textbf{0.8894±0.005}                                                                   & \textbf{0.6667±0.0002}                                                               & \textbf{0.688±0.0094}                                                               \\
                           & \begin{tabular}[c]{@{}l@{}}ImageNet \\ Transfer\end{tabular} & 0.8420±0.009                                                                   & 0.456±0.0077                                                                 & 0.6322±0.022      \\               

\midrule
\end{tabular}
\caption{Results for DINO, CASS, and Supervised (ImageNet-initialized transfer learning) methods on autoimmune biopsy slides, dermofit, and ISIC 2017 dataset. In this table, we compare the F1 score on the test set.}
\label{perf}
\end{table}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=1\textwidth]{image/overall.png}
    \caption{In this figure, we describe the overall process of medical image analysis. Passing the input image through the segmentation architecture yields a mask of foreground (pathology of interest) instead of the background (area other than the pathology of interest). Similarly, passing the same through a classifier (in green) yields a class prediction.}
\end{figure}



%%%%%Segmentation Table

 %Note: all reverse weight; 
\begin{table}[!htbp] 
        \begin{tabular}{c|ccccc}
            \toprule
             & \multicolumn{5}{c}{ \textbf{Percentage of Training data ($x \%$ labeled data)} } \\
             &$0 \%$  & $10 \%$  & 50\% & 70\% & $100 \%$  \\
            
            \midrule
             & \multicolumn{4}{c}{ \textbf{Dermofit Dataset (Interpolate to 480x480 then resize to 224x224)}} \\
            \midrule
            \textbf{PiCIE(Rn34)} &0.5698  &&&& \\
            \textbf{DEDL(Rn34)} & &0.6599  & 0.7198  & 0.7229  & 0.7576  \\
            \textbf{Semi-SL(ST)} & &\textbf{0.7244} & \textbf{0.7954} & \textbf{0.8033} & \textbf{0.8182 } \\
            % \textbf{SSL(Unet)} & 1 & 1 & 1 & 1\\
            
            \midrule  
             & \multicolumn{4}{c}{ \textbf{Dermatomyositis (Tilling to 480x480 then resize to 224x224) }} \\
            \midrule
            \textbf{PiCIE(Rn34)} &0.4151  &&&& \\
            \textbf{DEDL(Rn34)} & &0.4237  & 0.5261 & 0.5407  & 0.5306  \\
            \textbf{Semi-SL(ST)} & &\textbf{0.5106 } & \textbf{0.5338} & \textbf{0.555} & \textbf{0.5751 } \\
             
             \midrule
             & \multicolumn{4}{c}{ \textbf{ISIC-2017 (Interpolate to 480x480 then resize to 224x224) }} \\
            \midrule
            \textbf{PiCIE(Rn34)} &0.4514  &&&& \\
            \textbf{DEDL(Rn34)} & &\textbf{0.5857} & 0.6171  & 0.5951  & 0.6518  \\
            \textbf{Semi-SL(ST)} & &0.5712  & \textbf{0.6637 } & \textbf{0.6763} & \textbf{0.7062 } \\
            % \textbf{SSL(Unet)}      & 0.5174 $\pm$ 0.019 & 0.5543 $\pm$ 0.0284 & 0.5521 $\pm$ 0.0167 & 0.5456 $\pm$ 0.0134 \\
            \bottomrule
        \end{tabular}
        \caption{Comparison Between Fully, Semi and UnSupervised architectures. Here, Rn34 represents ResNet-34 while ST represents Swin-U-Net. Since \cite{picie2021} is an unsupervised approach, it does not require any labels for fine-tuning. Hence, we present results for PiCIE using ResNet-34 backbone under 0\% label fractions. We observe that the semi-supervised approach outperforms the fully-supervised approach by using 50\% fewer per image labels on all three datasets.} 
    \label{table: fullyvsSemi}
\end{table}
